The Transit Light Curve (TLC) Project. II. Two Transits of the Exoplanet OGLE-TR-111b

As part of our ongoing effort to measure exoplanet sizes and transit times with greater accuracy, we present I band observations of two transits of OGLE-TR-111b. The photometry has an accuracy of 0.15-0.20% and a cadence of 1-2 minutes. We derive a planetary radius of 1.067 +/- 0.054 Jupiter radii and a stellar radius of 0.831 +/- 0.031 solar radii. The uncertainties are dominated by errors in the photometry, rather than by systematic errors arising from uncertainties in the limb darkening function or the stellar mass. Both the stellar radius and the planetary radius are in agreement with theoretical expectations. The transit times are accurate to within 30 seconds, and allow us to refine the estimate of the mean orbital period: 4.0144479 +/- 0.0000041 days.

==> table1.tex <==
$ 2453787.637339 $  &  $ 1.00005 $  &  $ 0.00158 $ \\
$ 2453787.638531 $  &  $ 1.00090 $  &  $ 0.00152 $ \\
$ 2453787.639816 $  &  $ 1.00026 $  &  $ 0.00151 $ \\
$ 2453787.640973 $  &  $ 0.99965 $  &  $ 0.00156 $ \\
$ 2453787.642131 $  &  $ 0.99900 $  &  $ 0.00154 $ \\
$ 2453787.643288 $  &  $ 1.00153 $  &  $ 0.00155 $ \\
$ 2453787.644457 $  &  $ 1.00156 $  &  $ 0.00149 $ \\
$ 2453787.645615 $  &  $ 0.99915 $  &  $ 0.00149 $ \\
$ 2453787.646760 $  &  $ 1.00200 $  &  $ 0.00149 $ \\
$ 2453787.647930 $  &  $ 0.99984 $  &  $ 0.00149 $ \\
$ 2453787.649099 $  &  $ 1.00068 $  &  $ 0.00154 $ \\
$ 2453787.650256 $  &  $ 1.00195 $  &  $ 0.00158 $ \\
$ 2453787.651483 $  &  $ 1.00198 $  &  $ 0.00159 $ \\
$ 2453787.652652 $  &  $ 1.00009 $  &  $ 0.00155 $ \\
$ 2453787.653809 $  &  $ 1.00035 $  &  $ 0.00158 $ \\
$ 2453787.654967 $  &  $ 0.99920 $  &  $ 0.00159 $ \\
$ 2453787.656136 $  &  $ 0.99918 $  &  $ 0.00159 $ \\
$ 2453787.657305 $  &  $ 0.99632 $  &  $ 0.00155 $ \\
$ 2453787.658462 $  &  $ 0.99461 $  &  $ 0.00151 $ \\
$ 2453787.659620 $  &  $ 0.99333 $  &  $ 0.00154 $ \\
$ 2453787.660789 $  &  $ 0.99256 $  &  $ 0.00156 $ \\
$ 2453787.661946 $  &  $ 0.99198 $  &  $ 0.00154 $ \\
$ 2453787.663104 $  &  $ 0.98830 $  &  $ 0.00152 $ \\
$ 2453787.664261 $  &  $ 0.98645 $  &  $ 0.00152 $ \\
$ 2453787.665419 $  &  $ 0.98582 $  &  $ 0.00156 $ \\
$ 2453787.666588 $  &  $ 0.98654 $  &  $ 0.00156 $ \\
$ 2453787.667745 $  &  $ 0.98601 $  &  $ 0.00154 $ \\
$ 2453787.668903 $  &  $ 0.98712 $  &  $ 0.00156 $ \\
$ 2453787.670060 $  &  $ 0.98617 $  &  $ 0.00159 $ \\
$ 2453787.671218 $  &  $ 0.98083 $  &  $ 0.00155 $ \\
$ 2453787.672387 $  &  $ 0.98023 $  &  $ 0.00158 $ \\
$ 2453787.673544 $  &  $ 0.98379 $  &  $ 0.00156 $ \\
$ 2453787.674701 $  &  $ 0.98301 $  &  $ 0.00154 $ \\
$ 2453787.675871 $  &  $ 0.98448 $  &  $ 0.00155 $ \\
$ 2453787.677028 $  &  $ 0.98143 $  &  $ 0.00152 $ \\
$ 2453787.678185 $  &  $ 0.97903 $  &  $ 0.00149 $ \\
$ 2453787.679354 $  &  $ 0.98477 $  &  $ 0.00148 $ \\
$ 2453787.680512 $  &  $ 0.98380 $  &  $ 0.00151 $ \\
$ 2453787.681681 $  &  $ 0.98302 $  &  $ 0.00149 $ \\
$ 2453787.682838 $  &  $ 0.98021 $  &  $ 0.00149 $ \\
$ 2453787.684007 $  &  $ 0.98210 $  &  $ 0.00154 $ \\
$ 2453787.685165 $  &  $ 0.98409 $  &  $ 0.00154 $ \\
$ 2453787.686392 $  &  $ 0.98206 $  &  $ 0.00149 $ \\
$ 2453787.687561 $  &  $ 0.98126 $  &  $ 0.00148 $ \\
$ 2453787.688718 $  &  $ 0.98270 $  &  $ 0.00154 $ \\
$ 2453787.689876 $  &  $ 0.98112 $  &  $ 0.00155 $ \\
$ 2453787.691033 $  &  $ 0.97864 $  &  $ 0.00158 $ \\
$ 2453787.692202 $  &  $ 0.98350 $  &  $ 0.00156 $ \\
$ 2453787.693360 $  &  $ 0.98293 $  &  $ 0.00158 $ \\
$ 2453787.694517 $  &  $ 0.98312 $  &  $ 0.00156 $ \\
$ 2453787.695686 $  &  $ 0.98109 $  &  $ 0.00156 $ \\
$ 2453787.696844 $  &  $ 0.98103 $  &  $ 0.00158 $ \\
$ 2453787.698001 $  &  $ 0.98044 $  &  $ 0.00158 $ \\
$ 2453787.699170 $  &  $ 0.98323 $  &  $ 0.00154 $ \\
$ 2453787.700339 $  &  $ 0.98299 $  &  $ 0.00154 $ \\
$ 2453787.701497 $  &  $ 0.98137 $  &  $ 0.00152 $ \\
$ 2453787.702666 $  &  $ 0.97872 $  &  $ 0.00151 $ \\
$ 2453787.703823 $  &  $ 0.98061 $  &  $ 0.00152 $ \\
$ 2453787.704981 $  &  $ 0.97924 $  &  $ 0.00152 $ \\
$ 2453787.706138 $  &  $ 0.98239 $  &  $ 0.00151 $ \\
$ 2453787.715421 $  &  $ 0.98354 $  &  $ 0.00154 $ \\
$ 2453787.716590 $  &  $ 0.98273 $  &  $ 0.00154 $ \\
$ 2453787.717747 $  &  $ 0.98245 $  &  $ 0.00156 $ \\
$ 2453787.718916 $  &  $ 0.98361 $  &  $ 0.00158 $ \\
$ 2453787.720074 $  &  $ 0.98300 $  &  $ 0.00162 $ \\
$ 2453787.721243 $  &  $ 0.98358 $  &  $ 0.00162 $ \\
$ 2453787.722400 $  &  $ 0.98320 $  &  $ 0.00155 $ \\
$ 2453787.723558 $  &  $ 0.98109 $  &  $ 0.00151 $ \\
$ 2453787.724715 $  &  $ 0.98418 $  &  $ 0.00152 $ \\
$ 2453787.725884 $  &  $ 0.98367 $  &  $ 0.00152 $ \\
$ 2453787.727042 $  &  $ 0.98260 $  &  $ 0.00160 $ \\
$ 2453787.728199 $  &  $ 0.98105 $  &  $ 0.00154 $ \\
$ 2453787.729368 $  &  $ 0.98005 $  &  $ 0.00154 $ \\
$ 2453787.730526 $  &  $ 0.98184 $  &  $ 0.00151 $ \\
$ 2453787.731683 $  &  $ 0.98345 $  &  $ 0.00155 $ \\
$ 2453787.732852 $  &  $ 0.98398 $  &  $ 0.00148 $ \\
$ 2453787.734021 $  &  $ 0.98309 $  &  $ 0.00152 $ \\
$ 2453787.735179 $  &  $ 0.98190 $  &  $ 0.00152 $ \\
$ 2453787.736336 $  &  $ 0.98311 $  &  $ 0.00148 $ \\
$ 2453787.737494 $  &  $ 0.98163 $  &  $ 0.00149 $ \\
$ 2453787.738651 $  &  $ 0.98502 $  &  $ 0.00151 $ \\
$ 2453787.739808 $  &  $ 0.98388 $  &  $ 0.00156 $ \\
$ 2453787.740966 $  &  $ 0.98402 $  &  $ 0.00151 $ \\
$ 2453787.742123 $  &  $ 0.98299 $  &  $ 0.00152 $ \\
$ 2453787.743281 $  &  $ 0.98420 $  &  $ 0.00151 $ \\
$ 2453787.744450 $  &  $ 0.98806 $  &  $ 0.00151 $ \\
$ 2453787.745607 $  &  $ 0.98494 $  &  $ 0.00155 $ \\
$ 2453787.746765 $  &  $ 0.98332 $  &  $ 0.00155 $ \\
$ 2453787.747922 $  &  $ 0.98525 $  &  $ 0.00156 $ \\
$ 2453787.749080 $  &  $ 0.98642 $  &  $ 0.00155 $ \\
$ 2453787.750237 $  &  $ 0.98463 $  &  $ 0.00154 $ \\
$ 2453787.751406 $  &  $ 0.98616 $  &  $ 0.00152 $ \\
$ 2453787.752564 $  &  $ 0.98598 $  &  $ 0.00154 $ \\
$ 2453787.753721 $  &  $ 0.99047 $  &  $ 0.00149 $ \\
$ 2453787.754890 $  &  $ 0.99162 $  &  $ 0.00154 $ \\
$ 2453787.756175 $  &  $ 0.99682 $  &  $ 0.00154 $ \\
$ 2453787.757344 $  &  $ 0.99414 $  &  $ 0.00158 $ \\
$ 2453787.758501 $  &  $ 0.99377 $  &  $ 0.00154 $ \\
$ 2453787.759659 $  &  $ 0.99598 $  &  $ 0.00155 $ \\
$ 2453787.760828 $  &  $ 0.99781 $  &  $ 0.00160 $ \\
$ 2453787.761985 $  &  $ 0.99634 $  &  $ 0.00160 $ \\
$ 2453787.763143 $  &  $ 1.00097 $  &  $ 0.00160 $ \\
$ 2453787.764300 $  &  $ 1.00191 $  &  $ 0.00154 $ \\
$ 2453787.765458 $  &  $ 1.00049 $  &  $ 0.00162 $ \\
$ 2453787.766615 $  &  $ 1.00164 $  &  $ 0.00149 $ \\
$ 2453787.767773 $  &  $ 1.00343 $  &  $ 0.00152 $ \\
$ 2453787.768930 $  &  $ 1.00112 $  &  $ 0.00154 $ \\
$ 2453799.641129 $  &  $ 0.99841 $  &  $ 0.00344 $ \\
$ 2453799.642552 $  &  $ 1.00003 $  &  $ 0.00354 $ \\
$ 2453799.643710 $  &  $ 1.00148 $  &  $ 0.00356 $ \\
$ 2453799.644867 $  &  $ 0.99981 $  &  $ 0.00348 $ \\
$ 2453799.646036 $  &  $ 0.99810 $  &  $ 0.00314 $ \\
$ 2453799.647194 $  &  $ 1.00266 $  &  $ 0.00327 $ \\
$ 2453799.648351 $  &  $ 0.99990 $  &  $ 0.00316 $ \\
$ 2453799.649509 $  &  $ 1.00164 $  &  $ 0.00325 $ \\
$ 2453799.650666 $  &  $ 0.99943 $  &  $ 0.00311 $ \\
$ 2453799.651835 $  &  $ 1.00162 $  &  $ 0.00302 $ \\
$ 2453799.652992 $  &  $ 1.00391 $  &  $ 0.00288 $ \\
$ 2453799.654289 $  &  $ 0.99714 $  &  $ 0.00275 $ \\
$ 2453799.655342 $  &  $ 0.99978 $  &  $ 0.00265 $ \\
$ 2453799.656384 $  &  $ 1.00001 $  &  $ 0.00272 $ \\
$ 2453799.657426 $  &  $ 0.99952 $  &  $ 0.00279 $ \\
$ 2453799.658467 $  &  $ 1.00111 $  &  $ 0.00287 $ \\
$ 2453799.659509 $  &  $ 0.99860 $  &  $ 0.00283 $ \\
$ 2453799.660551 $  &  $ 1.00031 $  &  $ 0.00270 $ \\
$ 2453799.661604 $  &  $ 1.00040 $  &  $ 0.00284 $ \\
$ 2453799.662646 $  &  $ 1.00155 $  &  $ 0.00283 $ \\
$ 2453799.663687 $  &  $ 1.00061 $  &  $ 0.00282 $ \\
$ 2453799.664926 $  &  $ 0.99755 $  &  $ 0.00271 $ \\
$ 2453799.665967 $  &  $ 1.00142 $  &  $ 0.00262 $ \\
$ 2453799.667009 $  &  $ 0.99983 $  &  $ 0.00278 $ \\
$ 2453799.668051 $  &  $ 1.00039 $  &  $ 0.00265 $ \\
$ 2453799.669081 $  &  $ 0.99963 $  &  $ 0.00267 $ \\
$ 2453799.670123 $  &  $ 0.99986 $  &  $ 0.00272 $ \\
$ 2453799.671176 $  &  $ 1.00122 $  &  $ 0.00274 $ \\
$ 2453799.672218 $  &  $ 1.00094 $  &  $ 0.00276 $ \\
$ 2453799.673259 $  &  $ 0.99985 $  &  $ 0.00264 $ \\
$ 2453799.674301 $  &  $ 1.00054 $  &  $ 0.00258 $ \\
$ 2453799.675493 $  &  $ 0.99921 $  &  $ 0.00226 $ \\
$ 2453799.676419 $  &  $ 1.00366 $  &  $ 0.00231 $ \\
$ 2453799.677357 $  &  $ 1.00315 $  &  $ 0.00229 $ \\
$ 2453799.678283 $  &  $ 1.00031 $  &  $ 0.00236 $ \\
$ 2453799.679220 $  &  $ 1.00136 $  &  $ 0.00234 $ \\
$ 2453799.680146 $  &  $ 1.00206 $  &  $ 0.00237 $ \\
$ 2453799.681072 $  &  $ 1.00203 $  &  $ 0.00244 $ \\
$ 2453799.682010 $  &  $ 0.99989 $  &  $ 0.00234 $ \\
$ 2453799.682936 $  &  $ 0.99936 $  &  $ 0.00238 $ \\
$ 2453799.683862 $  &  $ 0.99998 $  &  $ 0.00231 $ \\
$ 2453799.685233 $  &  $ 1.00292 $  &  $ 0.00213 $ \\
$ 2453799.686101 $  &  $ 0.99984 $  &  $ 0.00220 $ \\
$ 2453799.686969 $  &  $ 1.00060 $  &  $ 0.00223 $ \\
$ 2453799.687849 $  &  $ 0.99768 $  &  $ 0.00212 $ \\
$ 2453799.688717 $  &  $ 0.99909 $  &  $ 0.00207 $ \\
$ 2453799.689863 $  &  $ 0.99789 $  &  $ 0.00174 $ \\
$ 2453799.690615 $  &  $ 1.00027 $  &  $ 0.00179 $ \\
$ 2453799.691368 $  &  $ 0.99996 $  &  $ 0.00182 $ \\
$ 2453799.692132 $  &  $ 0.99943 $  &  $ 0.00188 $ \\
$ 2453799.692884 $  &  $ 0.99868 $  &  $ 0.00191 $ \\
$ 2453799.693636 $  &  $ 1.00159 $  &  $ 0.00182 $ \\
$ 2453799.694389 $  &  $ 1.00040 $  &  $ 0.00184 $ \\
$ 2453799.695141 $  &  $ 0.99974 $  &  $ 0.00177 $ \\
$ 2453799.695905 $  &  $ 1.00111 $  &  $ 0.00188 $ \\
$ 2453799.696657 $  &  $ 0.99911 $  &  $ 0.00187 $ \\
$ 2453799.697635 $  &  $ 0.99943 $  &  $ 0.00202 $ \\
$ 2453799.698445 $  &  $ 0.99608 $  &  $ 0.00199 $ \\
$ 2453799.699256 $  &  $ 0.99632 $  &  $ 0.00198 $ \\
$ 2453799.700066 $  &  $ 0.99577 $  &  $ 0.00207 $ \\
$ 2453799.700876 $  &  $ 0.99487 $  &  $ 0.00210 $ \\
$ 2453799.701686 $  &  $ 0.99529 $  &  $ 0.00207 $ \\
$ 2453799.702485 $  &  $ 0.99246 $  &  $ 0.00203 $ \\
$ 2453799.703307 $  &  $ 0.99294 $  &  $ 0.00198 $ \\
$ 2453799.704117 $  &  $ 0.98921 $  &  $ 0.00197 $ \\
$ 2453799.704927 $  &  $ 0.98837 $  &  $ 0.00190 $ \\
$ 2453799.706299 $  &  $ 0.99022 $  &  $ 0.00179 $ \\
$ 2453799.707051 $  &  $ 0.98834 $  &  $ 0.00174 $ \\
$ 2453799.707803 $  &  $ 0.98773 $  &  $ 0.00172 $ \\
$ 2453799.708556 $  &  $ 0.98511 $  &  $ 0.00173 $ \\
$ 2453799.709308 $  &  $ 0.98313 $  &  $ 0.00178 $ \\
$ 2453799.710060 $  &  $ 0.98344 $  &  $ 0.00173 $ \\
$ 2453799.710813 $  &  $ 0.98565 $  &  $ 0.00175 $ \\
$ 2453799.711565 $  &  $ 0.98283 $  &  $ 0.00178 $ \\
$ 2453799.712317 $  &  $ 0.98669 $  &  $ 0.00176 $ \\
$ 2453799.713070 $  &  $ 0.98382 $  &  $ 0.00180 $ \\
$ 2453799.715269 $  &  $ 0.98153 $  &  $ 0.00179 $ \\
$ 2453799.716033 $  &  $ 0.98384 $  &  $ 0.00183 $ \\
$ 2453799.716797 $  &  $ 0.98567 $  &  $ 0.00181 $ \\
$ 2453799.717549 $  &  $ 0.98279 $  &  $ 0.00179 $ \\
$ 2453799.718301 $  &  $ 0.98098 $  &  $ 0.00178 $ \\
$ 2453799.719054 $  &  $ 0.98552 $  &  $ 0.00189 $ \\
$ 2453799.719806 $  &  $ 0.98250 $  &  $ 0.00179 $ \\
$ 2453799.720558 $  &  $ 0.98184 $  &  $ 0.00182 $ \\
$ 2453799.721311 $  &  $ 0.98407 $  &  $ 0.00189 $ \\
$ 2453799.722063 $  &  $ 0.98115 $  &  $ 0.00181 $ \\
$ 2453799.722931 $  &  $ 0.98179 $  &  $ 0.00185 $ \\
$ 2453799.723695 $  &  $ 0.97922 $  &  $ 0.00184 $ \\
$ 2453799.724447 $  &  $ 0.98291 $  &  $ 0.00184 $ \\
$ 2453799.725200 $  &  $ 0.98200 $  &  $ 0.00181 $ \\
$ 2453799.725952 $  &  $ 0.98208 $  &  $ 0.00186 $ \\
$ 2453799.726705 $  &  $ 0.98218 $  &  $ 0.00178 $ \\
$ 2453799.727457 $  &  $ 0.98251 $  &  $ 0.00175 $ \\
$ 2453799.728209 $  &  $ 0.98215 $  &  $ 0.00175 $ \\
$ 2453799.728962 $  &  $ 0.98035 $  &  $ 0.00182 $ \\
$ 2453799.729714 $  &  $ 0.98187 $  &  $ 0.00177 $ \\
$ 2453799.730594 $  &  $ 0.97902 $  &  $ 0.00175 $ \\
$ 2453799.731346 $  &  $ 0.98302 $  &  $ 0.00180 $ \\
$ 2453799.732098 $  &  $ 0.98331 $  &  $ 0.00177 $ \\
$ 2453799.732851 $  &  $ 0.98104 $  &  $ 0.00179 $ \\
$ 2453799.733603 $  &  $ 0.98271 $  &  $ 0.00177 $ \\
$ 2453799.734355 $  &  $ 0.98200 $  &  $ 0.00180 $ \\
$ 2453799.735108 $  &  $ 0.98290 $  &  $ 0.00184 $ \\
$ 2453799.735871 $  &  $ 0.98081 $  &  $ 0.00184 $ \\
$ 2453799.736612 $  &  $ 0.97989 $  &  $ 0.00184 $ \\
$ 2453799.737365 $  &  $ 0.97751 $  &  $ 0.00177 $ \\
$ 2453799.738233 $  &  $ 0.97588 $  &  $ 0.00175 $ \\
$ 2453799.738997 $  &  $ 0.98372 $  &  $ 0.00178 $ \\
$ 2453799.739760 $  &  $ 0.98507 $  &  $ 0.00184 $ \\
$ 2453799.740513 $  &  $ 0.97751 $  &  $ 0.00182 $ \\
$ 2453799.741265 $  &  $ 0.98064 $  &  $ 0.00190 $ \\
$ 2453799.742018 $  &  $ 0.98195 $  &  $ 0.00179 $ \\
$ 2453799.742770 $  &  $ 0.98069 $  &  $ 0.00177 $ \\
$ 2453799.743522 $  &  $ 0.97972 $  &  $ 0.00182 $ \\
$ 2453799.744286 $  &  $ 0.98008 $  &  $ 0.00184 $ \\
$ 2453799.745027 $  &  $ 0.98223 $  &  $ 0.00179 $ \\
$ 2453799.746184 $  &  $ 0.97989 $  &  $ 0.00180 $ \\
$ 2453799.746937 $  &  $ 0.98260 $  &  $ 0.00186 $ \\
$ 2453799.747689 $  &  $ 0.98437 $  &  $ 0.00179 $ \\
$ 2453799.748453 $  &  $ 0.98111 $  &  $ 0.00177 $ \\
$ 2453799.749205 $  &  $ 0.97703 $  &  $ 0.00178 $ \\
$ 2453799.749958 $  &  $ 0.97532 $  &  $ 0.00178 $ \\
$ 2453799.750721 $  &  $ 0.98002 $  &  $ 0.00179 $ \\
$ 2453799.751474 $  &  $ 0.98081 $  &  $ 0.00179 $ \\
$ 2453799.752215 $  &  $ 0.98371 $  &  $ 0.00178 $ \\
$ 2453799.752967 $  &  $ 0.98252 $  &  $ 0.00180 $ \\
$ 2453799.753823 $  &  $ 0.97965 $  &  $ 0.00186 $ \\
$ 2453799.754576 $  &  $ 0.98215 $  &  $ 0.00182 $ \\
$ 2453799.755328 $  &  $ 0.97995 $  &  $ 0.00186 $ \\
$ 2453799.756092 $  &  $ 0.97873 $  &  $ 0.00188 $ \\
$ 2453799.756844 $  &  $ 0.97823 $  &  $ 0.00184 $ \\
$ 2453799.757597 $  &  $ 0.98141 $  &  $ 0.00190 $ \\
$ 2453799.758361 $  &  $ 0.98204 $  &  $ 0.00190 $ \\
$ 2453799.759113 $  &  $ 0.97676 $  &  $ 0.00187 $ \\
$ 2453799.759865 $  &  $ 0.97973 $  &  $ 0.00184 $ \\
$ 2453799.760618 $  &  $ 0.98244 $  &  $ 0.00185 $ \\
$ 2453799.761509 $  &  $ 0.98329 $  &  $ 0.00181 $ \\
$ 2453799.762261 $  &  $ 0.98325 $  &  $ 0.00188 $ \\
$ 2453799.763014 $  &  $ 0.98327 $  &  $ 0.00180 $ \\
$ 2453799.763766 $  &  $ 0.98066 $  &  $ 0.00178 $ \\
$ 2453799.764518 $  &  $ 0.97895 $  &  $ 0.00178 $ \\
$ 2453799.765271 $  &  $ 0.98303 $  &  $ 0.00181 $ \\
$ 2453799.766023 $  &  $ 0.98375 $  &  $ 0.00180 $ \\
$ 2453799.766775 $  &  $ 0.98061 $  &  $ 0.00184 $ \\
$ 2453799.767528 $  &  $ 0.98077 $  &  $ 0.00183 $ \\
$ 2453799.768280 $  &  $ 0.97656 $  &  $ 0.00186 $ \\
$ 2453799.769032 $  &  $ 0.98201 $  &  $ 0.00196 $ \\
$ 2453799.769785 $  &  $ 0.98118 $  &  $ 0.00184 $ \\
$ 2453799.770537 $  &  $ 0.98139 $  &  $ 0.00184 $ \\
$ 2453799.771289 $  &  $ 0.98146 $  &  $ 0.00181 $ \\
$ 2453799.772042 $  &  $ 0.98205 $  &  $ 0.00180 $ \\
$ 2453799.772794 $  &  $ 0.98302 $  &  $ 0.00181 $ \\
$ 2453799.773546 $  &  $ 0.98307 $  &  $ 0.00180 $ \\
$ 2453799.774299 $  &  $ 0.98404 $  &  $ 0.00184 $ \\
$ 2453799.775063 $  &  $ 0.98066 $  &  $ 0.00184 $ \\
$ 2453799.775815 $  &  $ 0.98069 $  &  $ 0.00179 $ \\
$ 2453799.776567 $  &  $ 0.98146 $  &  $ 0.00177 $ \\
$ 2453799.777320 $  &  $ 0.98056 $  &  $ 0.00177 $ \\
$ 2453799.778072 $  &  $ 0.98368 $  &  $ 0.00178 $ \\
$ 2453799.778824 $  &  $ 0.97909 $  &  $ 0.00176 $ \\
$ 2453799.779577 $  &  $ 0.98244 $  &  $ 0.00180 $ \\
$ 2453799.780329 $  &  $ 0.98543 $  &  $ 0.00179 $ \\
$ 2453799.781093 $  &  $ 0.98280 $  &  $ 0.00186 $ \\
$ 2453799.781834 $  &  $ 0.98223 $  &  $ 0.00194 $ \\
$ 2453799.782598 $  &  $ 0.98152 $  &  $ 0.00187 $ \\
$ 2453799.783350 $  &  $ 0.98467 $  &  $ 0.00180 $ \\
$ 2453799.784415 $  &  $ 0.98176 $  &  $ 0.00176 $ \\
$ 2453799.785167 $  &  $ 0.98148 $  &  $ 0.00184 $ \\
$ 2453799.785931 $  &  $ 0.97978 $  &  $ 0.00178 $ \\
$ 2453799.786672 $  &  $ 0.98326 $  &  $ 0.00175 $ \\
$ 2453799.787436 $  &  $ 0.98577 $  &  $ 0.00175 $ \\
$ 2453799.788188 $  &  $ 0.98746 $  &  $ 0.00175 $ \\
$ 2453799.788940 $  &  $ 0.98723 $  &  $ 0.00184 $ \\
$ 2453799.789693 $  &  $ 0.98448 $  &  $ 0.00174 $ \\
$ 2453799.790445 $  &  $ 0.98290 $  &  $ 0.00179 $ \\
$ 2453799.791197 $  &  $ 0.98160 $  &  $ 0.00177 $ \\
$ 2453799.791950 $  &  $ 0.98430 $  &  $ 0.00176 $ \\
$ 2453799.792702 $  &  $ 0.98458 $  &  $ 0.00175 $ \\
$ 2453799.793454 $  &  $ 0.98642 $  &  $ 0.00177 $ \\
$ 2453799.794207 $  &  $ 0.98568 $  &  $ 0.00179 $ \\
$ 2453799.794959 $  &  $ 0.98799 $  &  $ 0.00176 $ \\
$ 2453799.795711 $  &  $ 0.98757 $  &  $ 0.00181 $ \\
$ 2453799.796475 $  &  $ 0.98822 $  &  $ 0.00176 $ \\
$ 2453799.797274 $  &  $ 0.99022 $  &  $ 0.00181 $ \\
$ 2453799.798096 $  &  $ 0.99095 $  &  $ 0.00181 $ \\
$ 2453799.798894 $  &  $ 0.99188 $  &  $ 0.00178 $ \\
$ 2453799.799705 $  &  $ 0.99298 $  &  $ 0.00189 $ \\
$ 2453799.800445 $  &  $ 0.99319 $  &  $ 0.00185 $ \\
$ 2453799.801198 $  &  $ 0.98942 $  &  $ 0.00178 $ \\
$ 2453799.801950 $  &  $ 0.99440 $  &  $ 0.00185 $ \\
$ 2453799.802702 $  &  $ 0.99458 $  &  $ 0.00180 $ \\
$ 2453799.803455 $  &  $ 0.99436 $  &  $ 0.00181 $ \\
$ 2453799.804277 $  &  $ 1.00019 $  &  $ 0.00191 $ \\
$ 2453799.805110 $  &  $ 1.00110 $  &  $ 0.00185 $ \\
$ 2453799.805932 $  &  $ 0.99684 $  &  $ 0.00185 $ \\
$ 2453799.806765 $  &  $ 1.00159 $  &  $ 0.00190 $ \\
$ 2453799.807714 $  &  $ 0.99831 $  &  $ 0.00199 $ \\
$ 2453799.808536 $  &  $ 0.99994 $  &  $ 0.00183 $ \\
$ 2453799.809358 $  &  $ 1.00033 $  &  $ 0.00191 $ \\
$ 2453799.810133 $  &  $ 1.00108 $  &  $ 0.00181 $ \\
$ 2453799.810886 $  &  $ 0.99917 $  &  $ 0.00181 $ \\
$ 2453799.811638 $  &  $ 0.99934 $  &  $ 0.00185 $ \\
$ 2453799.812437 $  &  $ 0.99811 $  &  $ 0.00183 $ \\
$ 2453799.838734 $  &  $ 1.00405 $  &  $ 0.00187 $ \\
$ 2453799.839498 $  &  $ 0.99805 $  &  $ 0.00184 $ \\
$ 2453799.840250 $  &  $ 0.99975 $  &  $ 0.00187 $ \\
$ 2453799.841014 $  &  $ 1.00119 $  &  $ 0.00196 $ \\
$ 2453799.841766 $  &  $ 0.99727 $  &  $ 0.00182 $ \\
$ 2453799.842530 $  &  $ 1.00252 $  &  $ 0.00180 $ \\
$ 2453799.843283 $  &  $ 1.00322 $  &  $ 0.00181 $ \\
$ 2453799.844035 $  &  $ 1.00128 $  &  $ 0.00193 $ \\
$ 2453799.844799 $  &  $ 1.00119 $  &  $ 0.00202 $ \\
$ 2453799.845540 $  &  $ 0.99637 $  &  $ 0.00200 $ \\
$ 2453799.846396 $  &  $ 1.00278 $  &  $ 0.00195 $ \\
$ 2453799.847148 $  &  $ 0.99828 $  &  $ 0.00197 $ \\
$ 2453799.847901 $  &  $ 0.99992 $  &  $ 0.00188 $ \\
$ 2453799.848653 $  &  $ 0.99754 $  &  $ 0.00200 $ \\
$ 2453799.849405 $  &  $ 0.99673 $  &  $ 0.00205 $ \\
$ 2453799.850158 $  &  $ 1.00239 $  &  $ 0.00196 $ \\
$ 2453799.850910 $  &  $ 0.99836 $  &  $ 0.00212 $ \\
$ 2453799.851662 $  &  $ 0.99797 $  &  $ 0.00196 $ \\
$ 2453799.852426 $  &  $ 0.99796 $  &  $ 0.00201 $ \\
$ 2453799.853179 $  &  $ 0.99791 $  &  $ 0.00196 $ \\
$ 2453799.853931 $  &  $ 0.99463 $  &  $ 0.00198 $ \\
$ 2453799.854683 $  &  $ 1.00017 $  &  $ 0.00221 $ \\
$ 2453799.855436 $  &  $ 0.99935 $  &  $ 0.00212 $ \\
$ 2453799.856188 $  &  $ 1.00427 $  &  $ 0.00230 $ \\
$ 2453799.856940 $  &  $ 1.00065 $  &  $ 0.00201 $ \\
$ 2453799.857693 $  &  $ 1.00389 $  &  $ 0.00214 $ \\
$ 2453799.858445 $  &  $ 1.00184 $  &  $ 0.00200 $ \\
$ 2453799.859197 $  &  $ 1.00200 $  &  $ 0.00210 $ \\
$ 2453799.859961 $  &  $ 0.99963 $  &  $ 0.00206 $ \\
$ 2453799.860714 $  &  $ 1.00649 $  &  $ 0.00209 $ \\
$ 2453799.861466 $  &  $ 1.00161 $  &  $ 0.00201 $ \\
$ 2453799.862218 $  &  $ 1.00047 $  &  $ 0.00215 $ \\
$ 2453799.862971 $  &  $ 1.00099 $  &  $ 0.00203 $ \\
$ 2453799.863723 $  &  $ 1.00277 $  &  $ 0.00196 $ \\
$ 2453799.864487 $  &  $ 1.00339 $  &  $ 0.00196 $ \\
$ 2453799.865228 $  &  $ 0.99966 $  &  $ 0.00207 $ \\
$ 2453799.865992 $  &  $ 1.00621 $  &  $ 0.00236 $ \\
$ 2453799.866744 $  &  $ 0.99795 $  &  $ 0.00229 $ \\
$ 2453799.867496 $  &  $ 1.00266 $  &  $ 0.00213 $ \\
$ 2453799.868249 $  &  $ 0.99607 $  &  $ 0.00217 $ \\
$ 2453799.869157 $  &  $ 0.99782 $  &  $ 0.00240 $ \\
$ 2453799.869967 $  &  $ 1.00339 $  &  $ 0.00267 $ \\
$ 2453799.870778 $  &  $ 0.99728 $  &  $ 0.00279 $ \\
$ 2453799.871588 $  &  $ 1.00107 $  &  $ 0.00280 $ \\
$ 2453799.872410 $  &  $ 1.00190 $  &  $ 0.00295 $ \\
$ 2453799.873231 $  &  $ 0.99917 $  &  $ 0.00230 $ \\
$ 2453799.874065 $  &  $ 0.99839 $  &  $ 0.00249 $ \\
$ 2453799.874956 $  &  $ 0.99979 $  &  $ 0.00238 $ \\
$ 2453799.875859 $  &  $ 1.00231 $  &  $ 0.00250 $ \\
$ 2453799.876750 $  &  $ 0.99776 $  &  $ 0.00239 $ \\
$ 2453799.877826 $  &  $ 1.00173 $  &  $ 0.00294 $ \\
$ 2453799.878706 $  &  $ 0.99518 $  &  $ 0.00277 $ \\
$ 2453799.879597 $  &  $ 0.99728 $  &  $ 0.00258 $ \\
$ 2453799.880431 $  &  $ 0.99723 $  &  $ 0.00244 $ \\
$ 2453799.881241 $  &  $ 0.99948 $  &  $ 0.00246 $ \\
$ 2453799.882040 $  &  $ 0.99916 $  &  $ 0.00239 $ \\
$ 2453799.882850 $  &  $ 0.99870 $  &  $ 0.00256 $ \\
$ 2453799.883672 $  &  $ 1.00299 $  &  $ 0.00280 $ \\
$ 2453799.884482 $  &  $ 0.99634 $  &  $ 0.00272 $ \\
$ 2453799.885292 $  &  $ 1.00306 $  &  $ 0.00346 $ \\
$ 2453799.886102 $  &  $ 1.00264 $  &  $ 0.00291 $ \\
$ 2453799.886924 $  &  $ 1.00227 $  &  $ 0.00328 $ \\
$ 2453799.887734 $  &  $ 0.99897 $  &  $ 0.00322 $ \\
$ 2453799.889546 $  &  $ 1.00115 $  &  $ 0.00522 $ \\
$ 2453799.891091 $  &  $ 1.00760 $  &  $ 0.00540 $ \\
$ 2453799.892410 $  &  $ 0.99990 $  &  $ 0.00405 $ \\
$ 2453799.893568 $  &  $ 0.99949 $  &  $ 0.00462 $ \\
$ 2453799.894725 $  &  $ 1.00000 $  &  $ 0.00386 $ \\
$ 2453799.895883 $  &  $ 1.00058 $  &  $ 0.00362 $ \\
$ 2453799.897040 $  &  $ 1.00312 $  &  $ 0.00344 $ \\
$ 2453799.898209 $  &  $ 0.99972 $  &  $ 0.00352 $ \\
$ 2453799.899367 $  &  $ 1.00097 $  &  $ 0.00356 $ \\
$ 2453799.900524 $  &  $ 0.99810 $  &  $ 0.00330 $ \\
$ 2453799.901693 $  &  $ 0.99928 $  &  $ 0.00338 $ \\
$ 2453799.902850 $  &  $ 0.99692 $  &  $ 0.00349 $ \\
$ 2453799.904008 $  &  $ 1.00271 $  &  $ 0.00356 $ \\

